Quasinormal-mode modeling and design in nonlinear nano-optics

Based on quasinormal-mode theory, we propose a novel approach enabling a deep analytical insight into the multi-parameter design and optimization of nonlinear photonic structures at subwavelength scale. A key distinction of our method from previous formulations relying on multipolar Mie-scattering expansions is that it directly exploits the natural resonant modes of the nanostructures, which provide the field enhancement to achieve significant nonlinear efficiency. Thanks to closed-form expression for the nonlinear overlap integral between the interacting modes, we illustrate the potential of our method with a two-order-of-magnitude boost of second harmonic generation in a semiconductor nanostructure, by engineering both the sign of $\chi^{(2)}$ at subwavelength scale and the structure of the pump beam.

==> biblio.tex <==
@article{Gehrsitz2000,
abstract = {The refractive indices of AlxGa1−xAs epitaxial layers are accurately determined below the band gap to wavelengths, $\lambda${\textless}3 $\mu$m. The layers are grown on GaAs substrates by molecular beam epitaxy metal organic and chemical vapor deposition with thicknesses ranging from 4 to 10 $\mu$m. They form improper waveguide structures with the GaAs substrate. The measurements are based on the excitation of the improper waveguide modes with grating couplers at 23 °C. The refractive indices of the layers are derived from the modal propagation constants in the range of 730 nm{\textless}$\lambda${\textless}830 nm with an estimated uncertainty of $\Delta$n=5×10−4. The temperature coefficient of the refractive index is investigated in the same spectral range. From the effective indices of the TE and TM modes, we derive the strain-induced birefringence and the elasto-optic coefficients. High-resolution x-ray diffraction is used to determine the strain of the layers. The layer compositions are obtained with inductively coupled plasma atomic emission spectroscopy. The measurement range of the refractive index is extended from the direct gap to $\lambda${\textless}3 $\mu$m by observing the Fabry-P{\{}{\'{e}}{\}}rot interference fringes of the transmission spectra of isolated layers. The measured values of the refractive index and the elasto-optic coefficient are compared to calculated data based on semiempirical models described in the literature. Published data of the index of refraction on GaAs, AlAs and GaP are analyzed to permit the development of a modified Sellmeier approximation. The experimental data on AlxGa1−xAs can be fitted over the entire composition range 0⩽x⩽1 to provide an accurate analytical description as a function of composition, wavelength, and temperature. {\textcopyright} 2000 American Institute of Physics.},
author = {Gehrsitz, S. and Reinhart, F. K. and Gourgon, C. and Herres, N. and Vonlanthen, A. and Sigg, H.},
doi = {10.1063/1.373462},
file = {:C$\backslash$:/Users/DONNonlinearWS01/Desktop/PhD/Bibliography/Pool/1.373462.pdf:pdf},
issn = {00218979},
journal = {Journal of Applied Physics},
number = {11},
pages = {7825--7837},
title = {{The refractive index of AlxGa1-xAs below the band gap: Accurate determination and empirical modeling}},
volume = {87},
year = {2000}
}
@article{Kauranen2012,
abstract = {This chapter overviews nonlinear effects in plasmonics. A discussion of how to create linear and nonlinear surface plasmon-polaritons is presented, and is coupled to a basic discussion of third-harmonic generation. The generation of nonlinear surface plasmon-polaritons is then discussed not only in terms of third-harmonic generation but as a consequence of the breaking of translational symmetry in a conventional interface system. The evolution of polaritons into solitons is highlighted. A detailed review of nonlinear plasmonics is then given that includes field enhancement of localized surface plasmons and controlling light with light. Switching and modulation of surface plasmon-polariton signals are then reviewed. After a discussion of nonlinear plasmonic crystals, and structured metal surfaces, some comments on metamaterials are also included. It is emphasized that nonlinear plasmonics will have an invaluable impact on future conventional and quantum nanophotonic technologies.},
archivePrefix = {arXiv},
arxivId = {1312.6806},
author = {Kauranen, M. and Zayats, A. V.},
doi = {10.1038/NPHOTON.2012.244},
eprint = {1312.6806},
file = {:C$\backslash$:/Users/DONNonlinearWS01/AppData/Local/Mendeley Ltd./Mendeley Desktop/Downloaded/Kauranen, Zayats - 2012 - Nonlinear plasmonics.pdf:pdf},
isbn = {1749-4885$\backslash$r1749-4893},
issn = {15734331},
journal = {Nature Photonics},
keywords = {Harmonics,Nonlinear plasmonics,Plasmons,Polaritons,Switching,Technology},
number = {October},
pages = {737--748},
pmid = {23389280},
publisher = {Nature Publishing Group},
title = {{Nonlinear plasmonics}},
url = {http://dx.doi.org/10.1038/nphoton.2012.244},
volume = {4},
year = {2012}
}
@article{Kuo2006,
abstract = {We have generated an ultrabroad mid-infrared continuum by using single-pass optical parametric generation (OPG) in orientation-patterned GaAs (OP-GaAs). The spectrum spans more than an octave, from 4.5 to 10.7 microm, measured 20 dB down from the peak. The 17.5 mm long, 0.5 mm thick, all-epitaxially-grown OP-GaAs sample with a 166.6-microm quasi-phase-matching period was pumped with 3.1-3.3 microm wavelength, 1 ps pulses up to 2 microJ in energy. The OPG threshold was observed at 55 nJ pump energy with the pump polarized along the [111] crystal direction. The slope efficiency near threshold was 51{\%}, and the external conversion efficiency was as high as 15{\%}.},
author = {Kuo, P. S. and Vodopyanov, K. L. and Fejer, M. M. and Simanovskii, D. M. and Yu, X. and Harris, J. S. and Bliss, D. and Weyburne, D.},
doi = {10.1364/ol.31.000071},
file = {:C$\backslash$:/Users/DONNonlinearWS01/Desktop/PhD/Bibliography/Pool/ol-31-1-71.pdf:pdf},
issn = {0146-9592},
journal = {Optics Letters},
number = {1},
pages = {71--73},
title = {{Optical parametric generation of a mid-infrared continuum in orientation-patterned GaAs}},
volume = {31},
year = {2006}
}
@article{Bautista2018,
abstract = {{\textcopyright} 2018 American Chemical Society. We investigate collective effects in plasmonic oligomers of different symmetries using second-harmonic generation (SHG) microscopy with cylindrical vector beams (CVBs). The oligomers consist of gold nanorods that have a longitudinal plasmon resonance close to the fundamental wavelength that is used for SHG excitation and whose long axes are arranged locally such that they follow the distribution of the transverse component of the electric field of radially or azimuthally polarized CVBs in the focal plane. We observe that SHG from such rotationally symmetric oligomers is strongly modified by the interplay between the polarization properties of the CVB and interparticle coupling. We find that the oligomers with radially oriented nanorods exhibit small coupling effects. In contrast, we find that the oligomers with azimuthally oriented nanorods exhibit large coupling effects that lead to silencing of SHG from the whole structure. Our experimental results are in very good agreement with numerical calculations based on the boundary element method. The work describes a new route for studying coupling effects in complex arrangements of nano-objects and thereby for tailoring the efficiency of nonlinear optical effects in such structures.},
author = {Bautista, Godofredo and Dreser, Christoph and Zang, Xiaorun and Kern, Dieter P. and Kauranen, Martti and Fleischer, Monika},
doi = {10.1021/acs.nanolett.8b00308},
file = {:C$\backslash$:/Users/DONNonlinearWS01/Desktop/PhD/Bibliography/Pool/acs.nanolett.8b00308.pdf:pdf},
issn = {15306992},
journal = {Nano Letters},
keywords = {1 here,attention in recent years,boundary element method,cylindrical vector beams,electron beam lithography,metal nanoparticles,onlinear plasmonics has been,plasmonic oligomers,receiving widespread,second-harmonic generation microscopy},
number = {4},
pages = {2571--2580},
publisher = {American Chemical Society},
title = {{Collective Effects in Second-Harmonic Generation from Plasmonic Oligomers}},
volume = {18},
year = {2018}
}
@article{Carletti2016,
abstract = {We study the manipulation of the radiation pattern of second-harmonic generation from AlGaAs all-dielectric nanoantennas exhibiting electric and magnetic resonances. We show the importance of the interference of different higher order multipoles in the nonlinear response of dielectric antennas for shaping of their second-harmonic radiation pattern. In particular, we show how such multipolar interference can be engineered in AlGaAs nanodisks by manipulating the pump beam polarization, incidence angle, and disk geometry. In this way we demonstrate the shaping of the radiation pattern in order to increase the second-harmonic power by a factor of 8 when measured in experiment through a finite numerical aperture microscope objective.},
author = {Carletti, Luca and Locatelli, Andrea and Neshev, Dragomir and {De Angelis}, Costantino},
doi = {10.1021/acsphotonics.6b00050},
file = {:C$\backslash$:/Users/DONNonlinearWS01/Desktop/PhD/Bibliography/Pool/acsphotonics.6b00050.pdf:pdf},
issn = {23304022},
journal = {ACS Photonics},
keywords = {nanoantennas,nonlinear scattering,radiation pattern,second-harmonic generation},
number = {8},
pages = {1500--1507},
title = {{Shaping the Radiation Pattern of Second-Harmonic Generation from AlGaAs Dielectric Nanoantennas}},
volume = {3},
year = {2016}
}
@article{Krischek2010,
abstract = {Ultrafast, ultraviolet light pulses are a key tool for spectroscopic studies (for example, molecular formation1, 2 and carrier dynamics in semiconductors3) as well as a source for non-classical states of light4, 5, 6, 7, 8, 9, 10, 11, 12, 13. The power required for many nonlinear processes makes amplifier systems mandatory, which significantly reduces the available repetition rate and thus often lengthens the experimental acquisition time. Here we adopt techniques recently developed for the infrared regime14, 15, 16 to design the first enhancement cavity for femtosecond ultraviolet pulses. An average ultraviolet power of more than 7W at a repetition rate of 81MHz is now available to pump a nonlinear crystal inside the cavity, applied here to implement a powerful source for high-rate experiments with entangled multiphoton states. The field enhancement enables a new scale of experiments in photonic quantum logic and in nonlinear optics research, for example, to operate optical parametric amplifiers at high repetition rates or to create high-harmonic-frequency combs14, 15, 16.},
author = {Krischek, Roland and Wieczorek, Witlef and Ozawa, Akira and Kiesel, Nikolai and Michelberger, Patrick and Udem, Thomas and Weinfurter, Harald},
doi = {10.1038/nphoton.2009.286},
file = {:C$\backslash$:/Users/DONNonlinearWS01/Desktop/PhD/Bibliography/Pool/nphoton.2009.286.pdf:pdf},
issn = {17494885},
journal = {Nature Photonics},
number = {3},
pages = {170--173},
publisher = {Nature Publishing Group},
title = {{Ultraviolet enhancement cavity for ultrafast nonlinear optics and high-rate multiphoton entanglement experiments}},
volume = {4},
year = {2010}
}
@article{DeLong1994,
abstract = {We discuss the use of second-harmonic generation (SHG) as the nonlinearity in the technique of frequency- resolved optical gating (FROG) for measuring the full intensity and phase evolution of an arbitrary ultrashort pulse. FROG that uses a third-order nonlinearity in the polarization-gate geometry has proved extremely successful, and the algorithm required for extraction of the intensity and the phase from the experimental data is quite robust. However, for pulse intensities less than -1 MW, third-order nonlinearities generate insuffi- cient signal strength, and therefore SHG FROG appears necessary. We discuss the theoretical, algorithmic, and experimental considerations of SHG FROG in detail. SHG FROG has an ambiguity in the direction of time, and its traces are somewhat unintuitive. Also, previously published algorithms are generally ineffective at extracting the intensity and the phase of an arbitrary laser pulse from the SHG FROG trace. We present an improved pulse-retrieval algorithm, based on the method of generalized projections, that is far superior to the previously published algorithms, although it is still not so robust as the polarization-gate algorithm. We discuss experimental sources of error such as pump depletion and group-velocity mismatch. We also present several experimental examples of pulses measured with SHG FROG and show that the derived intensities and phases are in agreement with more conventional diagnostic techniques, and we demonstrate the high- dynamic-range capability of SHG FROG. We conclude that, despite the above drawbacks, SHG FROG should be useful in measuring low-energy pulses. 1.},
author = {DeLong, K. W. and Trebino, Rick and Hunter, J. and White, W. E.},
doi = {10.1364/josab.11.002206},
file = {:C$\backslash$:/Users/DONNonlinearWS01/Desktop/PhD/Bibliography/Pool/josab-11-11-2206.pdf:pdf},
issn = {0740-3224},
journal = {Journal of the Optical Society of America B},
number = {11},
pages = {2206--2215},
title = {{Frequency-resolved optical gating with the use of second-harmonic generation}},
volume = {11},
year = {1994}
}
@article{Guasoni2017,
abstract = {We develop a novel theoretical model for the study of harmonic generation in cylindrical structures of finite height. Our technique is based on the decomposition of the electromagnetic field over the complete set of modes of the corresponding infinite cylinder. Differently from previous works, in our model no constraints are given neither on the cross section nor on the refractive index of the cylinder. We then apply our approach in the special case of frequency doubling in tall AlGaAs nanodisks, where radiative modes can be neglected. Our results open new perspectives for optimization and engineering of the radiation pattern in harmonic generation processes at the nanoscale.},
author = {Guasoni, Massimiliano and Carletti, Luca and Neshev, Dragomir and {De Angelis}, Costantino},
doi = {10.1109/JQE.2017.2697973},
file = {:C$\backslash$:/Users/DONNonlinearWS01/Desktop/PhD/Bibliography/Pool/guasoni2017.pdf:pdf},
issn = {00189197},
journal = {IEEE Journal of Quantum Electronics},
keywords = {Subwavelength structures,harmonic generation and mixing},
number = {3},
pages = {1--5},
title = {{Theoretical Model for Pattern Engineering of Harmonic Generation in All-Dielectric Nanoantennas}},
volume = {53},
year = {2017}
}
@article{Arbore1997,
abstract = {We demonstrate the use of an aperiodic quasi-phase-matching (QPM) grating to generate second-harmonic pulses that are stretched or compressed relative to input pulses at the fundamental frequency. We frequency doubled an externally chirped erbium-doped fiber laser generating 17-ps (FWHM) pulses at 1560nm to produce near-transform-limited 110-fs (FWHM) pulses at 780nm by use of a 5-cm-long lithium niobate crystal poled with a QPM grating chirped from an 18.2- to a 19.8-microm period.},
author = {Arbore, M. A. and Galvanauskas, A. and Harter, D. and Chou, M. H. and Fejer, M. M.},
doi = {10.1364/ol.22.001341},
file = {:C$\backslash$:/Users/DONNonlinearWS01/Desktop/PhD/Bibliography/Pool/120.pdf:pdf},
issn = {0146-9592},
journal = {Optics Letters},
number = {17},
pages = {1341--1343},
title = {{Engineerable compression of ultrashort pulses by use of second-harmonic generation in chirped-period-poled lithium niobate}},
volume = {22},
year = {1997}
}
@article{Heinz1982,
author = {Heinz, T F and Chen, C K and Ricard, D. and Shen, Y.R.},
file = {:C$\backslash$:/Users/DONNonlinearWS01/Desktop/PhD/Bibliography/Pool/PhysRevLett.48.478.pdf:pdf},
number = {7},
pages = {478--481},
title = {{Spectroscopy of Molecular Monolayers by Resonant Second-Harmonic Generation}},
volume = {48},
year = {1982}
}
@article{Shcherbakov2015,
abstract = {We demonstrate experimentally ultrafast alloptical switching in subwavelength nonlinear dielectric nanostructures exhibiting localized magnetic Mie resonances. We employ amorphous silicon nanodisks to achieve strong self-modulation of femtosecond pulses with a depth of 60{\%} at picojoule-per-disk pump energies. In the pump−probe measurements, we reveal that switching in the nanodisks can be governed by pulse-limited 65 fs-long two-photon absorption being enhanced by a factor of 80 with respect to the unstructured silicon film. We also show that undesirable free-carrier effects can be suppressed by a proper spectral positioning of the magnetic resonance, making such a structure the fastest all-optical switch operating at the nanoscale.},
author = {Shcherbakov, Maxim R. and Vabishchevich, Polina P. and Shorokhov, Alexander S. and Chong, Katie E. and Choi, Duk Yong and Staude, Isabelle and Miroshnichenko, Andrey E. and Neshev, Dragomir N. and Fedyanin, Andrey A. and Kivshar, Yuri S.},
doi = {10.1021/acs.nanolett.5b02989},
file = {:C$\backslash$:/Users/DONNonlinearWS01/AppData/Local/Mendeley Ltd./Mendeley Desktop/Downloaded/Shcherbakov et al. - 2015 - Ultrafast All-Optical Switching with Magnetic Resonances in Nonlinear Dielectric Nanostructures.pdf:pdf;:C$\backslash$:/Users/DONNonlinearWS01/AppData/Local/Mendeley Ltd./Mendeley Desktop/Downloaded/Shcherbakov et al. - 2015 - Ultrafast All-Optical Switching with Magnetic Resonances in Nonlinear Dielectric Nanostructures(2).pdf:pdf},
isbn = {1530-6984},
issn = {15306992},
journal = {Nano Letters},
keywords = {Nonlinear optics,all-optical switching,femtosecond optics,metasurfaces,optical magnetism,silicon photonics},
number = {10},
pages = {6985--6990},
pmid = {26393983},
title = {{Ultrafast All-Optical Switching with Magnetic Resonances in Nonlinear Dielectric Nanostructures}},
volume = {15},
year = {2015}
}
@article{Almeida2016,
abstract = {A hologram is an optical element storing phase and possibly amplitude information enabling the reconstruction of a three dimensional image of an object by illumination and scattering of a coherent beam of light, and the image is generated at the same wavelength as the input laser beam. In recent years it was shown that information can be stored in nanometric antennas giving rise to ultrathin components. Here we demonstrate nonlinear multi-layer metamaterial holograms where by the nonlinear process of Third Harmonic Generation, a background free image is formed at a new frequency which is the third harmonic of the illuminating beam. Using e-beam lithography of multilayer plasmonic nanoantennas, we fabricate polarization-sensitive nonlinear elements such as blazed gratings, lenses and other computer-generated holograms. These holograms are analyzed and prospects for future device applications are discussed.},
archivePrefix = {arXiv},
arxivId = {1512.07899},
author = {Almeida, Euclides and Bitton, Ora and Prior, Yehiam},
doi = {10.1038/ncomms12533},
eprint = {1512.07899},
file = {:C$\backslash$:/Users/DONNonlinearWS01/AppData/Local/Mendeley Ltd./Mendeley Desktop/Downloaded/Almeida, Bitton, Prior - 2016 - Nonlinear metamaterials for holography.pdf:pdf},
isbn = {9788578110796},
issn = {20411723},
journal = {Nature Communications},
pages = {1--7},
pmid = {25246403},
title = {{Nonlinear metamaterials for holography}},
volume = {7},
year = {2016}
}
@article{Kruk2017,
abstract = {{\textcopyright} 2017 American Chemical Society. Nonlinear effects at the nanoscale are usually associated with the enhancement of electric fields in plasmonic structures. Recently emerged new platform for nanophotonics based on high-index dielectric nanoparticles utilizes optically induced magnetic response via multipolar Mie resonances and provides novel opportunities for nanoscale nonlinear optics. Here, we observe strong second-harmonic generation from AlGaAs nanoantennas driven by both electric and m agnetic resonances. We distinguish experimentally the contribution of electric and magnetic nonlinear response by analyzing the structure of polarization states of vector beams in the second-harmonic radiation. We control continuously the transition between electric and magnetic nonlinearities by tuning polarization of the optical pump. Our results provide a direct observation of nonlinear optical magnetism through selective excitation of multipolar nonlinear modes in nanoantennas.},
author = {Kruk, Sergey S. and Camacho-Morales, Rocio and Xu, Lei and Rahmani, Mohsen and Smirnova, Daria A. and Wang, Lei and Tan, Hark Hoe and Jagadish, Chennupati and Neshev, Dragomir N. and Kivshar, Yuri S.},
doi = {10.1021/acs.nanolett.7b01488},
file = {:C$\backslash$:/Users/DONNonlinearWS01/Desktop/PhD/Bibliography/Pool/acs.nanolett.7b01488.pdf:pdf},
issn = {15306992},
journal = {Nano Letters},
keywords = {Nonlinear nanophotonics,dielectric nanoantennas,nanofabrication,optical magnetism,second-harmonic generation,semiconductors},
number = {6},
pages = {3914--3918},
title = {{Nonlinear optical magnetism revealed by second-harmonic generation in nanoantennas}},
volume = {17},
year = {2017}
}
@article{Colom2018,
author = {Colom, R{\'{e}}mi and McPhedran, Ross and Stout, Brian and Bonod, Nicolas},
doi = {10.1103/PhysRevB.98.085418},
file = {:C$\backslash$:/Users/DONNonlinearWS01/Desktop/PhD/Bibliography/Pool/PhysRevB.98.085418.pdf:pdf},
issn = {24699969},
journal = {Physical Review B},
keywords = {doi:10.1103/PhysRevB.98.085418 url:https://doi.org},
number = {8},
pages = {1--5},
publisher = {American Physical Society},
title = {{Modal expansion of the scattered field: Causality, nondivergence, and nonresonant contribution}},
volume = {98},
year = {2018}
}
@article{Kivshar2018,
author = {Kivshar, Yuri},
doi = {10.1093/nsr/nwy017},
file = {:C$\backslash$:/Users/DONNonlinearWS01/AppData/Local/Mendeley Ltd./Mendeley Desktop/Downloaded/Kivshar - 2018 - All-dielectric meta-optics and nonlinear nanophotonics.pdf:pdf},
issn = {2095-5138},
journal = {National Science Review},
keywords = {meta-optics,metamaterials,metasurfaces,mie resonances,nanophotonics},
number = {January},
pages = {144--158},
title = {{All-dielectric meta-optics and nonlinear nanophotonics}},
url = {http://academic.oup.com/nsr/advance-article/doi/10.1093/nsr/nwy017/4822169},
year = {2018}
}
@article{Celebrano2015,
abstract = {Boosting nonlinear frequency conversion in extremely confined volumes remains a key challenge in nano-optics, nanomedicine, photocatalysis, and background-free biosensing. To this aim, field enhancements in plasmonic nanostructures are often exploited to effectively compensate for the lack of phase-matching at the nanoscale. Second harmonic generation (SHG) is, however, strongly quenched by the high degree of symmetry in plasmonic materials at the atomic scale and in nanoantenna designs. Here, we devise a plasmonic nanoantenna lacking axial symmetry, which exhibits spatial and frequency mode overlap at both the excitation and the SHG wavelengths. The effective combination of these features in a single device allows obtaining unprecedented SHG conversion efficiency. Our results shed new light on the optimization of SHG at the nanoscale, paving the way to new classes of nanoscale coherent light sources and molecular sensing devices based on nonlinear plasmonic platforms.},
archivePrefix = {arXiv},
arxivId = {1412.0698},
author = {Celebrano, Michele and Wu, Xiaofei and Baselli, Milena and Gro{\ss}mann, Swen and Biagioni, Paolo and Locatelli, Andrea and {De Angelis}, Costantino and Cerullo, Giulio and Osellame, Roberto and Hecht, Bert and Du{\`{o}}, Lamberto and Ciccacci, Franco and Finazzi, Marco},
doi = {10.1038/nnano.2015.69},
eprint = {1412.0698},
file = {:C$\backslash$:/Users/DONNonlinearWS01/AppData/Local/Mendeley Ltd./Mendeley Desktop/Downloaded/Celebrano et al. - 2015 - Mode matching in multiresonant plasmonic nanoantennas for enhanced second harmonic generation.pdf:pdf},
isbn = {1748-3395 (Electronic)
1748-3387 (Linking)},
issn = {17483395},
journal = {Nature Nanotechnology},
number = {5},
pages = {412--417},
pmid = {25895003},
publisher = {Nature Publishing Group},
title = {{Mode matching in multiresonant plasmonic nanoantennas for enhanced second harmonic generation}},
url = {http://dx.doi.org/10.1038/nnano.2015.69},
volume = {10},
year = {2015}
}
@article{Shcherbakov2015a,
abstract = {It is known that the nonlinear optical properties of photonic nanostructures can be modified substantially due to strong field confinement and optical resonances. In this contribution, we study third-harmonic generation from low-loss subwavelength silicon nanodisks arranged in the form of trimer oligomers with varying distance between the nanoparticles. Each of the nanodisks exhibits both electric and magnetic Mie-type resonances that are shown to affect significantly the nonlinear response. We observe the third-harmonic radiation intensity that is comparable to that of a bulk silicon slab and demonstrate a pronounced reshaping of the third-harmonic spectra due to interference of the nonlinearly generated waves augmented by an interplay between the electric and the magnetic dipolar resonances.$\backslash$nIt is known that the nonlinear optical properties of photonic nanostructures can be modified substantially due to strong field confinement and optical resonances. In this contribution, we study third-harmonic generation from low-loss subwavelength silicon nanodisks arranged in the form of trimer oligomers with varying distance between the nanoparticles. Each of the nanodisks exhibits both electric and magnetic Mie-type resonances that are shown to affect significantly the nonlinear response. We observe the third-harmonic radiation intensity that is comparable to that of a bulk silicon slab and demonstrate a pronounced reshaping of the third-harmonic spectra due to interference of the nonlinearly generated waves augmented by an interplay between the electric and the magnetic dipolar resonances.},
author = {Shcherbakov, Maxim R. and Shorokhov, Alexander S. and Neshev, Dragomir N. and Hopkins, Ben and Staude, Isabelle and Melik-Gaykazyan, Elizaveta V. and Ezhov, Alexander A. and Miroshnichenko, Andrey E. and Brener, Igal and Fedyanin, Andrey A. and Kivshar, Yuri S.},
doi = {10.1021/acsphotonics.5b00065},
file = {:C$\backslash$:/Users/DONNonlinearWS01/AppData/Local/Mendeley Ltd./Mendeley Desktop/Downloaded/Shcherbakov et al. - 2015 - Nonlinear interference and tailorable third-harmonic generation from dielectric oligomers.pdf:pdf},
issn = {23304022},
journal = {ACS Photonics},
keywords = {Mie scattering,nanoparticle oligomers,nonlinear optics,optical magnetism,silicon nanoparticles,third-harmonic generation},
number = {5},
pages = {578--582},
title = {{Nonlinear interference and tailorable third-harmonic generation from dielectric oligomers}},
volume = {2},
year = {2015}
}
@article{More1971,
abstract = {This paper constructs a special perturbation theory vrhich directly describes the alteration of decaying states by an external perturbation. The complex energies of the decaying states appear in this theory. When lifetime effects are taken into account, we find that the criteria for quantum degeneracy are slightly strengthened and sharpened. We also discuss the smooth merger of the properties of decaying states and those of true eigenstates in the case of long lifetimes.},
author = {More, R. M.},
doi = {10.1103/PhysRevA.4.1782},
file = {:C$\backslash$:/Users/DONNonlinearWS01/Desktop/PhD/Bibliography/Pool/PhysRevA.4.1782.pdf:pdf},
issn = {10502947},
journal = {Physical Review A},
number = {5},
pages = {1782--1790},
title = {{Theory of decaying states}},
volume = {4},
year = {1971}
}
@article{Tanzilli2005,
abstract = {Quantum communication is the art of transferring quantum states, or quantum bits of information (qubits), from one place to another. On the fundamental side, this allows one to distribute entanglement and demonstrate quantum nonlocality over significant distances. On the more applied side, quantum cryptography offers, for the first time in human history, a provably secure way to establish a confidential key between distant partners. Photons represent the natural flying qubit carriers for quantum communication, and the presence of telecom optical fibres makes the wavelengths of 1310 and 1550 nm particulary suitable for distribution over long distances. However, to store and process quantum information, qubits could be encoded into alkaline atoms that absorb and emit at around 800 nm wavelength. Hence, future quantum information networks made of telecom channels and alkaline memories will demand interfaces able to achieve qubit transfers between these useful wavelengths while preserving quantum coherence and entanglement. Here we report on a qubit transfer between photons at 1310 and 710 nm via a nonlinear up-conversion process with a success probability greater than 5{\%}. In the event of a successful qubit transfer, we observe strong two-photon interference between the 710 nm photon and a third photon at 1550 nm, initially entangled with the 1310 nm photon, although they never directly interacted. The corresponding fidelity is higher than 98{\%}.},
author = {Tanzilli, S. and Tittel, W. and Halder, M. and Alibart, O. and Baldi, P. and Gisin, N. and Zbinden, H.},
doi = {10.1038/nature04009},
file = {:C$\backslash$:/Users/DONNonlinearWS01/Desktop/PhD/Bibliography/Pool/nature04009.pdf:pdf},
issn = {14764687},
journal = {Nature},
number = {7055},
pages = {116--120},
title = {{A photonic quantum information interface}},
volume = {437},
year = {2005}
}
@inproceedings{Hughes2019,
author = {Hughes, Tyler W. and Minkov, Momchil and Williamson, Ian A. D. and Fan, Shanhui},
booktitle = {Conference on Lasers and Electro-Optics, OSA Technical Digest (Optical Society of America, 2019), paper SW4J.7},
title = {{Adjoint-based inverse design of nonlinear nanophotonic devices}},
year = {2019}
}
@article{Camacho-Morales2016,
abstract = {The quest for nanoscale light sources with designer radiation patterns and polarization has motivated the development of nanoantennas that interact strongly with the incoming light and are able to transform its frequency, radiation and polarization patterns. Here, we demonstrate dielectric AlGaAs nanoantennas for efficient second harmonic generation, enabling the control of both directionality and polarization of nonlinear emission. This is enabled by specialized III-V semiconductor nanofabrication of high-quality AlGaAs nanostructures embedded in optically transparent low-index material, thus allowing for simultaneous forward and backward nonlinear emission. We show that the nanodisk AlGaAs antennas can emit second harmonic in preferential direction with backward-to-forward ratio up to five, as well as can generate complex vector polarization beams, including beams with radial polarization.},
author = {Camacho-Morales, Rocio and Rahmani, Mohsen and Kruk, Sergey and Wang, Lei and Xu, Lei and Smirnova, Daria A. and Solntsev, Alexander S. and Miroshnichenko, Andrey and Tan, Hark Hoe and Karouta, Fouad and Naureen, Shagufta and Vora, Kaushal and Carletti, Luca and {De Angelis}, Costantino and Jagadish, Chennupati and Kivshar, Yuri S. and Neshev, Dragomir N.},
doi = {10.1021/acs.nanolett.6b03525},
file = {:C$\backslash$:/Users/DONNonlinearWS01/AppData/Local/Mendeley Ltd./Mendeley Desktop/Downloaded/Camacho-Morales et al. - 2016 - Nonlinear Generation of Vector Beams from AlGaAs Nanoantennas.pdf:pdf},
isbn = {1530-6992 (Electronic)
1530-6984 (Linking)},
issn = {15306992},
journal = {Nano Letters},
keywords = {III-V semiconductors,Nonlinear optics,dielectric nanoantennas,nanofabrication,nanophotonics,second harmonic generation},
number = {11},
pages = {7191--7197},
pmid = {27797212},
title = {{Nonlinear Generation of Vector Beams from AlGaAs Nanoantennas}},
volume = {16},
year = {2016}
}
@article{Lalanne2018,
abstract = {In this Review, the theory and applications of optical micro and nanoresonators are presented from the underlying concept of their natural resonances, the so-called quasi-normal modes (QNMs). The latter are the basic constituents governing the response of resonators. Characterized by complex frequencies, QNMs are initially loaded by a driving field and then decay exponentially in time due to power leakage or absorption. Here, the use of QNM-expansion formalisms to model these basic effects is explored. Such modal expansions that operate at complex frequencies distinguish from the current user habits in electromagnetic modeling, which rely on classical Maxwell equation solvers operating at real frequencies or in the time domain; they also bring much deeper physical insight into the analysis. An extensive overview of the historical background on QNMs in electromagnetism and a detailed discussion of recent relevant theoretical and numerical advances are therefore presented. Additionally, a concise description of the role of QNMs on a number of examples involving electromagnetic resonant fields and matter, including the interaction between quantum emitters and resonators (Purcell effect, weak and strong coupling, superradiance...), Fano interferences, the perturbation of resonance modes, and light transport and localization in disordered media is provided.},
author = {Lalanne, Philippe and Yan, Wei and Vynck, Kevin and Sauvan, Christophe and Hugonin, Jean Paul},
doi = {10.1002/lpor.201700113},
file = {:C$\backslash$:/Users/DONNonlinearWS01/AppData/Local/Mendeley Ltd./Mendeley Desktop/Downloaded/Lalanne et al. - 2018 - Light Interaction with Photonic and Plasmonic Resonances.pdf:pdf},
issn = {18638899},
journal = {Laser and Photonics Reviews},
keywords = {Fano resonance,LDOS,cavity perturbation theory,electromagnetic resonance,microcavities,mode volumes,nanoantennas},
number = {5},
pages = {1--38},
title = {{Light Interaction with Photonic and Plasmonic Resonances}},
volume = {12},
year = {2018}
}
@article{Leung1994,
abstract = {It is shown that for the scalar analog of electrodynamics in one dimension, the quasinormal modes of a leaky cavity form a complete set inside the cavity, provided the cavity is defined by a discontinuity in the refractive index. This condition is sufficiently general to apply to a number of interesting examples. The quasinormal modes are also orthogonal under a modified definition of the inner product. The complete- ness and orthogonality hold even though the cavity is not a Hermitian system by itself. These properties allow the discrete quasinormal modes to be used as the basis for dynamics of the scalar wave in the cavi- ty.},
author = {Leung, P T and Liu, S Y and Young, K},
file = {:C$\backslash$:/Users/DONNonlinearWS01/Desktop/PhD/Bibliography/Pool/PhysRevA.49.3057.pdf:pdf},
journal = {Physical Review A},
number = {4},
pages = {3057--3067},
title = {{Completeness and orthogonahty of qnaslnormal modes xn leaky optical cavities}},
url = {https://journals.aps.org/pra/pdf/10.1103/PhysRevA.49.3057},
volume = {49},
year = {1994}
}
@article{Eyres2001,
abstract = {Orientation-patterned GaAs (OPGaAs) films of 200 $\mu$m thickness have been grown by hydride vapor phase epitaxy (HVPE) on an orientation-patterned template fabricated by molecular beam epitaxy (MBE). Fabrication of the templates utilized only MBE and chemical etching, taking advantage of GaAs/Ge/GaAs heteroepitaxy to control the crystal orientation of the top GaAs film relative to the substrate. Antiphase domain boundaries were observed to propagate vertically under HVPE growth conditions so that the domain duty cycle was preserved through the thick GaAs for all domain periods attempted. Quasiphase-matched frequency doubling of a CO2 laser was demonstrated with the beam confocally focused through a 4.6 mm long OPGaAs film. {\textcopyright} 2001 American Institute of Physics.},
author = {Eyres, L. A. and Tourreau, P. J. and Pinguet, T. J. and Ebert, C. B. and Harris, J. S. and Fejer, M. M. and Becouarn, L. and Gerard, B. and Lallier, E.},
doi = {10.1063/1.1389326},
file = {:C$\backslash$:/Users/DONNonlinearWS01/AppData/Local/Mendeley Ltd./Mendeley Desktop/Downloaded/Eyres et al. - 2001 - All-epitaxial fabrication of thick, orientation-patterned GaAs films for nonlinear optical frequency conversion.pdf:pdf},
issn = {00036951},
journal = {Applied Physics Letters},
number = {7},
pages = {904--906},
title = {{All-epitaxial fabrication of thick, orientation-patterned GaAs films for nonlinear optical frequency conversion}},
volume = {79},
year = {2001}
}
@article{Vodopyanov2004,
abstract = {We demonstrate a GaAs based OPO. The singly-resonant, pulsed OPO utilized an all-epitaxially-grown orientation-patterned GaAs (OP-GaAs) crystal. By tuning either near-IR pump wavelength or OP-GaAs temperature, we achieved broad tunability between 2 and 10 microns. {\textcopyright} 2001 Optical Society of America.},
author = {Vodopyanov, K. L. and Levi, O. and Kuo, P. S. and Pinguet, T. J. and Harris, J. S. and Fejer, M. M. and Gerard, B. and Becouara, L. and Lallier, E.},
doi = {10.1364/ol.29.001912},
file = {:C$\backslash$:/Users/DONNonlinearWS01/Desktop/PhD/Bibliography/Pool/ol-29-16-1912.pdf:pdf},
isbn = {9781628414370},
issn = {10945695},
journal = {OSA Trends in Optics and Photonics Series},
number = {16},
pages = {459--461},
title = {{Optical parametric oscillation in quasi-phasematched GaAs}},
volume = {96 A},
year = {2004}
}
@article{Oron2008,
abstract = {Material preparation methods and device fabrication technologies for realization of low loss periodically oriented GaAs waveguides are reported. Planar waveguide structures were grown by MOCVD on periodically patterned templates prepared by wafer bonding and selective layer removal. Ridge waveguides were designed and fabricated from the planar structures with emphasis on waveguide loss minimization. Record low losses of 2.0db/cm in periodically oriented waveguides and 0.95db/cm in single domain waveguides were measured. Routes for further loss reduction in patterned GaAs waveguides are discussed and initial results from further work to reduce waveguide corrugation are presented.},
author = {Oron, M. B. and Shusterman, S. and Blau, P.},
doi = {10.1117/12.758646},
file = {:C$\backslash$:/Users/DONNonlinearWS01/Desktop/PhD/Bibliography/Pool/oron2008.pdf:pdf},
isbn = {9780819470508},
issn = {0277786X},
journal = {Nonlinear Frequency Generation and Conversion: Materials, Devices, and Applications VII},
keywords = {frequency conversion,mocvd regrowth,op-gaas template,op-gaas waveguide,opo,periodically oriented gaas,quasi phase matching,second harmonic generation,waveguide,waveguide loss},
pages = {1--12},
title = {{Periodically oriented GaAs templates and waveguide structures for frequency conversion}},
volume = {6875},
year = {2008}
}
@article{Wu2019,
abstract = {We introduce a theoretical and computational method to design resonant objects, such as nanoantennas or meta-atoms, exhibiting tailored multipolar responses. In contrast with common approaches that rely on a multipolar analysis of the scattering response of an object upon specific excitations, we propose to engineer the intrinsic (i.e., excitation-independent) multipolar content and spectral characteristics of the natural resonances -- or quasinormal modes -- of the object. A rigorous numerical approach for the multipolar decomposition of resonances at complex frequencies is presented, along with an analytical model conveying a direct physical insight into the multipole moments induced in the resonator. Our design strategy is illustrated by designing a subwavelength optical resonator exhibiting a Janus resonance that provides side-dependent coupling to waveguides over the full linewidth of the resonance and on a wide angular range for linearly-polarized incident planewaves. The method applies to all kinds of waves and may open new perspectives for subwavelength-scale manipulation of scattering and emission.},
archivePrefix = {arXiv},
arxivId = {1907.04598},
author = {Wu, Tong and Baron, Alexandre and Lalanne, Philippe and Vynck, Kevin},
eprint = {1907.04598},
file = {:C$\backslash$:/Users/DONNonlinearWS01/Desktop/PhD/Bibliography/Pool/1907.04598.pdf:pdf},
journal = {arxiv},
title = {{Intrinsic multipolar contents of nanoresonators for tailored scattering}},
url = {http://arxiv.org/abs/1907.04598},
year = {2019}
}
@article{Rodriguez2007,
author = {Rodriguez, Alejandro and Soljacic, Marin and Joannopoulos, J D and Johnson, Steven G},
file = {:C$\backslash$:/Users/DONNonlinearWS01/Desktop/PhD/Bibliography/Pool/oe-15-12-7303.pdf:pdf},
journal = {Optics Express},
number = {12},
pages = {7303--7318},
title = {$\chi$(2) and $\chi$(3) harmonic generation at a critical power in inhomogeneous doubly resonant cavities},
volume = {15},
year = {2007}
}
@article{Smirnova2016,
abstract = {Nonlinear nanophotonics is a rapidly developing field with many useful applications for a design of nonlinear nanoantennas, light sources, nanolasers, sensors, and ultrafast miniature metadevices. A tight confinement of the local electromagnetic fields in resonant photonic nanostructures can boost nonlinear optical effects, thus offering versatile opportunities for subwavelength control of light. To achieve the desired functionalities, it is essential to gain flexible control over the near- and far-field properties of nanostructures. Thus, both modal and multipolar analyses are widely exploited for engineering nonlinear scattering from resonant nanoscale elements, in particular for enhancing the near-field interaction, tailoring the far-field multipolar interference, and optimization of the radiation directionality. Here, we review the recent advances in this recently emerged research field ranging from metallic structures exhibiting localized plasmonic resonances to hybrid metal-dielectric and all-dielectric nanostructures driven by Mie-type multipolar resonances and optically-induced magnetic response.},
archivePrefix = {arXiv},
arxivId = {1609.02057},
author = {Smirnova, Daria and Kivshar, Yuri S.},
doi = {10.1364/OPTICA.3.001241},
eprint = {1609.02057},
file = {:C$\backslash$:/Users/DONNonlinearWS01/AppData/Local/Mendeley Ltd./Mendeley Desktop/Downloaded/Smirnova, Kivshar - 2016 - Multipolar nonlinear nanophotonics.pdf:pdf},
issn = {2334-2536},
journal = {Optica},
number = {11},
pages = {1241--1252},
title = {{Multipolar nonlinear nanophotonics}},
url = {http://arxiv.org/abs/1609.02057{\%}0Ahttp://dx.doi.org/10.1364/OPTICA.3.001241},
volume = {3},
year = {2016}
}
@article{Berger1998,
abstract = {In this paper, we describe a theoretical approach by which we can qualitatively and quantitatively determine the nonlinear optical properties of a photonic crystals. We start by accurately characterizing the linear properties of the structure, using a recently developed multigrid method to efficiently compute the photonic bandstructure and Bloch functions of the PC. This results in a generalization of the slowly varying envelope approximation to the case of nonlinear PCs. {\textcopyright} 2003 IEEE.},
author = {Berger, V.},
doi = {10.1109/CLEOE.2003.1312311},
file = {:C$\backslash$:/Users/DONNonlinearWS01/Desktop/PhD/Bibliography/Pool/PhysRevLett.81.4136.pdf:pdf},
isbn = {0780377346},
issn = {10797114},
journal = {Physical Review Letters},
number = {19},
pages = {4136--4139},
title = {{Nonlinear photonic crystals}},
volume = {81},
year = {1998}
}
@article{Yan2018,
abstract = {The specificity of modal-expansion formalisms is their capabilities to model the physical properties in the natural resonance-state basis of the system in question, leading to a transparent interpretation of the numerical results. In electromagnetism, modal-expansion formalisms are routinely used for optical waveguides. In contrast, they are much less mature for analyzing open non-Hermitian systems, such as micro and nanoresonators. Here, by accounting for material dispersion with auxiliary fields, we considerably extend the capabilities of these formalisms, in terms of computational effectiveness, number of states handled and range of validity. We implement an efficient finite element solver to compute the resonance states, and derive new closed-form expressions of the modal excitation coefficients for reconstructing the scattered fields. Together, these two achievements allow us to perform rigorous modal analysis of complicated plasmonic resonators, being not limited to a few resonance states, with straightforward physical interpretations and remarkable computation speeds. We particularly show that, when the number of states retained in the expansion increases, convergence towards accurate predictions is achieved, offering a solid theoretical foundation for analyzing important issues, e.g. Fano interference, quenching, coupling with the continuum, which are critical in nanophotonic research.},
author = {Yan, Wei and Faggiani, R{\'{e}}mi and Lalanne, Philippe},
doi = {10.1103/PhysRevB.97.205422},
file = {:C$\backslash$:/Users/DONNonlinearWS01/AppData/Local/Mendeley Ltd./Mendeley Desktop/Downloaded/Yan, Faggiani, Lalanne - 2018 - Rigorous modal analysis of plasmonic nanoresonators.pdf:pdf},
issn = {24699969},
journal = {Physical Review B},
number = {20},
pages = {205422 1--9},
title = {{Rigorous modal analysis of plasmonic nanoresonators}},
volume = {97},
year = {2018}
}
@article{Vial2014,
abstract = {A quasimodal expansion method (QMEM) is developed to model and understand the scattering properties of arbitrary shaped two-dimensional (2-D) open structures. In contrast with the bounded case which have only discrete spectrum (real in the lossless media case), open resonators show a continuous spectrum composed of radiation modes and may also be characterized by resonances associated to complex eigenvalues (quasimodes). The use of a complex change of coordinates to build Perfectly Matched Layers (PMLs) allows the numerical computation of those quasimodes and of approximate radiation modes. Unfortunately, the transformed operator at stake is no longer self-adjoint, and classical modal expansion fails. To cope with this issue, we consider an adjoint eigenvalue problem which eigenvectors are bi-orthogonal to the eigenvectors of the initial problem. The scattered field is expanded on this complete set of modes leading to a reduced order model of the initial problem. The different contributions of the eigenmodes to the scattered field unambiguously appears through the modal coefficients, allowing us to analyze how a given mode is excited when changing incidence parameters. This gives new physical insights to the spectral properties of different open structures such as nanoparticles and diffraction gratings. Moreover, the QMEM proves to be extremely efficient for the computation of Local Density Of States (LDOS).},
author = {Vial, Benjamin and Zolla, Fr{\'{e}}d{\'{e}}ric and Nicolet, Andr{\'{e}} and Commandr{\'{e}}, Mireille},
doi = {10.1103/PhysRevA.89.023829},
file = {:C$\backslash$:/Users/DONNonlinearWS01/Desktop/PhD/Bibliography/Pool/PhysRevA.89.023829.pdf:pdf},
issn = {10502947},
journal = {Physical Review A - Atomic, Molecular, and Optical Physics},
number = {2},
pages = {1--15},
title = {{Quasimodal expansion of electromagnetic fields in open two-dimensional structures}},
volume = {89},
year = {2014}
}
@article{Lin2016,
author = {Lin, Zin and Liang, Xiangdong and Lon{\v{c}}ar, Marko and Johnson, Steven G. and Rodriguez, Alejandro W.},
doi = {10.1364/OPTICA.3.000233},
file = {:C$\backslash$:/Users/DONNonlinearWS01/Desktop/PhD/Bibliography/Pool/2016 Optica S Johnson interessant.pdf:pdf},
issn = {2334-2536},
journal = {Optica},
number = {3},
pages = {233--238},
title = {{Cavity-enhanced second-harmonic generation via nonlinear-overlap optimization}},
url = {https://www.osapublishing.org/abstract.cfm?URI=optica-3-3-233},
volume = {3},
year = {2016}
}
@article{Powell2017,
abstract = {The modes of silicon meta-atoms are investigated, motivated by their use as building blocks of Huygens' metasurfaces. A model based on these modes is presented, giving a clear physical explanation of all features in the extinction spectrum. Counter-intuitively, this can show negative contributions to extinction, which are shown to arise from the interference between non-orthogonal modes. The direct and interference contributions to extinction are determined, showing that conservation of energy is preserved. The Huygens' condition of matched electric and magnetic dipole moments leads to strong forward scattering and suppressed back scattering. It is shown that higher order modes with appropriate symmetry generalise this condition, leading to multiple bands of directional scattering. The presented results are obtained using a robust approach to find the modes of nano-photonic scatterers, commonly referred to as quasi-normal modes. By utilising an integral formulation of Maxwell's equations, this work avoids the problem of normalising diverging far-fields, which other approaches require. The model and presented results are implemented in open-source code.},
author = {Powell, David A.},
doi = {10.1103/PhysRevApplied.7.034006},
file = {:C$\backslash$:/Users/DONNonlinearWS01/Desktop/PhD/Bibliography/Pool/PhysRevApplied.7.034006.pdf:pdf},
issn = {23317019},
journal = {Physical Review Applied},
number = {3},
pages = {1--13},
title = {{Interference between the Modes of an All-Dielectric Meta-atom}},
volume = {7},
year = {2017}
}
@article{Sauvan2013,
abstract = {We provide a self-consistent electromagnetic theory of the coupling between dipole emitters and dissipative nanoresonators. The theory that relies on the concept of quasinormal modes with complex frequencies provides an accurate closed-form expression for the electromagnetic local density of states of any photonic or plasmonic resonator with strong radiation leakage, absorption, and material dispersion. It represents a powerful tool to calculate and conceptualize the electromagnetic response of systems that are governed by a small number of resonance modes. We use the formalism to revisit Purcell's factor. The new formula substantially differs from the usual one; in particular, it predicts that a spectral detuning between the emitter and the resonance does not necessarily result in a Lorentzian response in the presence of dissipation. Comparisons with fully vectorial numerical calculations for plasmonic nanoresonators made of gold nanorods evidence the high accuracy of the predictions achieved by our semianalytical treatment. {\textcopyright} 2013 American Physical Society.},
author = {Sauvan, C. and Hugonin, J. P. and Maksymov, I. S. and Lalanne, P.},
doi = {10.1103/PhysRevLett.110.237401},
file = {:C$\backslash$:/Users/DONNonlinearWS01/Desktop/PhD/Bibliography/Pool/PhysRevLett.110.237401.pdf:pdf},
issn = {00319007},
journal = {Physical Review Letters},
number = {23},
pages = {1--5},
title = {{Theory of the spontaneous optical emission of nanosize photonic and plasmon resonators}},
volume = {110},
year = {2013}
}
@article{Yang2016,
abstract = {Light emitters or scatterers embedded in stratified media may couple energy to both free-space modes and guided modes of the stratified structure. For a comprehensive analysis, it is important to evaluate the angular intensity distribution of both the free-space modes and guided modes excited in such systems. In the present work, we propose an original method based on Lorentz reciprocity theorem to efficiently calculate the free-space and guided radiation diagrams with a high accuracy from the sole knowledge of the near-field around the emitters or scatterers. Compared to conventional near-to-far field transformation techniques, the proposal allows one to easily evaluate the guided-mode radiation diagrams, even if material dissipation is present in the stack, and thus to simultaneously track the coupling of light to all channels (i.e., free-space and guided ones). We also provide an open-source code that may be used with essentially any Maxwell's equation solver. The numerical tool may help to engineer various devices, such as light-emitting diodes or nanoantennas, to achieve directional and efficient radiative spontaneous decays in free-space and guided optics.},
author = {Yang, Jianji and Hugonin, Jean Paul and Lalanne, Philippe},
doi = {10.1021/acsphotonics.5b00559},
file = {:C$\backslash$:/Users/DONNonlinearWS01/Desktop/PhD/Bibliography/Pool/acsphotonics.5b00559.pdf:pdf},
issn = {23304022},
journal = {ACS Photonics},
keywords = {Lorentz reciprocity,computational electrodynamics,light emission,light scattering,mode expansion,radiation diagram,stratified structure},
number = {3},
pages = {395--402},
title = {{Near-to-Far Field Transformations for Radiative and Guided Waves}},
volume = {3},
year = {2016}
}
@article{Yang2015,
abstract = {{\textcopyright} 2015 American Chemical Society. We derive a closed-form expression that accurately predicts the peak frequency shift and broadening induced by tiny perturbations of plasmonic nanoresonators without critically relying on repeated electrodynamic simulations of the spectral response of nanoresonator for various locations, sizes, or shapes of the perturbing objects. In comparison with other approaches of the same kind, the force of the present approach is that the derivation is supported by a mathematical formalism based on a rigorous normalization of the resonance modes of nanoresonators consisting of lossy and dispersive materials. Accordingly, accurate predictions are obtained for a large range of nanoparticle shapes and sizes used in various plasmonic nanosensors even beyond the quasistatic limit. The expression gives quantitative insight and, combined with an open-source code, provides accurate and fast predictions that are ideally suited for preliminary designs or for interpretation of experimental data. It is also valid for photonic resonators with large mode volumes.},
author = {Yang, Jianji and Giessen, Harald and Lalanne, Philippe},
doi = {10.1021/acs.nanolett.5b00771},
file = {:C$\backslash$:/Users/DONNonlinearWS01/Desktop/PhD/Bibliography/Pool/acs.nanolett.5b00771.pdf:pdf},
issn = {15306992},
journal = {Nano Letters},
keywords = {Refractive index sensing,nanoparticle,plasmonics,quasi normal mode,surface plasmon resonance},
number = {5},
pages = {3439--3444},
title = {{Simple analytical expression for the peak-frequency shifts of plasmonic resonances for sensing}},
volume = {15},
year = {2015}
}
@article{Ilchenko2004,
abstract = {We demonstrate parametric frequency doubling in a whispering gallery cavity made of periodically poled lithium niobate. This demonstration is an example of utility of such crystalline optical whispering gallery resonators with very high [Formula presented] factors, which we have fabricated. {\textcopyright} 2004 The American Physical Society.},
author = {Ilchenko, Vladimir S. and Savchenkov, Anatoliy A. and Matsko, Andrey B. and Maleki, Lute},
doi = {10.1103/PhysRevLett.92.043903},
file = {:C$\backslash$:/Users/DONNonlinearWS01/Desktop/PhD/Bibliography/Pool/PhysRevLett.92.043903.pdf:pdf},
issn = {10797114},
journal = {Physical Review Letters},
number = {4},
pages = {1--4},
title = {{Nonlinear Optics and Crystalline Whispering Gallery Mode Cavities}},
volume = {92},
year = {2004}
}
@article{Notomi2010,
abstract = {Recently, strongly modulated photonic crystals, fabricated by the state-of-the-art semiconductor nanofabrication process, have realized various novel optical properties. This paper describes the way in which they differ from other optical media, and clarifies what they can do. In particular, three important issues are considered: light confinement, frequency dispersion and spatial dispersion. First, I describe the latest status and impact of ultra-strong light confinement in a wavelength-cubic volume achieved in photonic crystals. Second, the extreme reduction in the speed of light is reported, which was achieved as a result of frequency dispersion management. Third, strange negative refraction in photonic crystals is introduced, which results from their unique spatial dispersion, and it is clarified how this leads to perfect imaging. The last two sections are devoted to applications of these novel properties. First, I report the fact that strong light confinement and huge light–matter interaction enhancement make strongly modulated photonic crystals promising for on-chip all-optical processing, and present several examples including all-optical switches/memories and optical logics. As a second application, it is shown that the strong light confinement and slow light in strongly modulated photonic crystals enable the adiabatic tuning of light, which leads to various novel ways of controlling light, such as adiabatic frequency conversion, efficient optomechanics systems, photon memories and photons pinning.},
author = {Notomi, Masaya},
doi = {10.1088/0034-4885/73/9/096501},
file = {:C$\backslash$:/Users/DONNonlinearWS01/Desktop/PhD/Bibliography/Pool/Notomi{\_}2010{\_}Rep.{\_}Prog.{\_}Phys.{\_}73{\_}096501.pdf:pdf},
issn = {00344885},
journal = {Reports on Progress in Physics},
number = {9},
pages = {1--57},
title = {{Manipulating light with strongly modulated photonic crystals}},
volume = {73},
year = {2010}
}
@article{Doost2014,
abstract = {The resonant state expansion (RSE), a rigorous perturbative method in electrodynamics, is developed for three-dimensional open optical systems. Results are presented using the analytically solvable homogeneous dielectric sphere as unperturbed system. Since any perturbation which breaks the spherical symmetry mixes transverse electric (TE) and transverse magnetic (TM) modes, the RSE is extended here to include TM modes and a zero-frequency pole of the Green's function. We demonstrate the validity of the RSE for TM modes by verifying its convergence towards the exact result for a homogeneous perturbation of the sphere. We then apply the RSE to calculate the modes for a selection of perturbations sequentially reducing the remaining symmetry, given by a change of the dielectric constant of half-sphere and quarter-sphere shape. Since no exact solutions are known for these perturbations, we verify the RSE results by comparing them with the results of state of the art finite element method (FEM) and finite difference in time domain (FDTD) solvers. We find that for the selected perturbations, the RSE provides a significantly higher accuracy than the FEM and FDTD for a given computational effort, demonstrating its potential to supersede presently used methods. We furthermore show that in contrast to presently used methods, the RSE is able to determine the perturbation of a selected group of modes by using a limited basis local to these modes, which can further reduce the computational effort by orders of magnitude.},
author = {Doost, M. B. and Langbein, W. and Muljarov, E. A.},
doi = {10.1103/PhysRevA.90.013834},
file = {:C$\backslash$:/Users/DONNonlinearWS01/Desktop/PhD/Bibliography/Pool/PhysRevA.90.013834.pdf:pdf},
issn = {10941622},
journal = {Physical Review A - Atomic, Molecular, and Optical Physics},
number = {1},
pages = {1--14},
title = {{Resonant-state expansion applied to three-dimensional open optical systems}},
volume = {90},
year = {2014}
}
@article{Frizyuk2019,
abstract = {We develop a multipolar theory of second-harmonic generation (SHG) by dielectric nanoparticles made of noncentrosymmetric materials with bulk quadratic nonlinearity. We specifically analyze two regimes of optical excitation: illumination by a plane wave and single-mode excitation, when the laser pump drives the magnetic dipole mode only. Considering two classes of nonlinear crystalline solids (dielectric perovskite material and III-V semiconductor), we apply a symmetry approach to derive selection rules for the multipolar composition of the nonlinear radiation. The developed description can be used for design of efficient nonlinear optical nanoantennas with reconfigurable radiation characteristics.},
author = {Frizyuk, Kristina and Volkovskaya, Irina and Smirnova, Daria and Poddubny, Alexander and Petrov, Mihail},
doi = {10.1103/PhysRevB.99.075425},
file = {:C$\backslash$:/Users/DONNonlinearWS01/AppData/Local/Mendeley Ltd./Mendeley Desktop/Downloaded/Frizyuk et al. - 2019 - Second-harmonic generation in Mie-resonant dielectric nanoparticles made of noncentrosymmetric materials.pdf:pdf},
issn = {24699969},
journal = {Physical Review B},
keywords = {doi:10.1103/PhysRevB.99.075425 url:https://doi.org},
number = {7},
pages = {1--15},
publisher = {American Physical Society},
title = {{Second-harmonic generation in Mie-resonant dielectric nanoparticles made of noncentrosymmetric materials}},
volume = {99},
year = {2019}
}
@article{Sehmi2017,
abstract = {Approximating the frequency dispersion of the permittivity of materials with simple analytical functions is of fundamental importance for understanding and modeling their optical properties. Quite generally, the permittivity can be treated in the complex frequency plane as an analytic function having a countable number of simple poles which determine the dispersion of the permittivity, with the pole weights corresponding to generalized conductivities of the medium at these resonances. The resulting Drude-Lorentz model separates the poles at frequencies with zero real part (Ohm's law and Drude poles) from poles with finite real part (Lorentz poles). To find the parameters of such an analytic function, we minimize the error weighted deviation between the model and measured values of the permittivity. We show examples of such optimizations for various semiconductors (Si, GaAs and Ge), for different frequency ranges and up to five pairs of Lorentz poles accounted for in the model.},
archivePrefix = {arXiv},
arxivId = {arXiv:1705.05218v1},
author = {Sehmi, H. S. and Langbein, W. and Muljarov, E. A.},
doi = {10.1109/PIERS.2017.8261889},
eprint = {arXiv:1705.05218v1},
file = {:C$\backslash$:/Users/DONNonlinearWS01/Desktop/PhD/Bibliography/Pool/1705.05218.pdf:pdf},
isbn = {9781509062690},
issn = {19317360},
journal = {Progress in Electromagnetics Research Symposium},
pages = {994--1000},
title = {{Optimizing the drude-lorentz model for material permittivity: Examples for semiconductors}},
year = {2017}
}
@article{Veysi2016,
abstract = {An azimuthally E-polarized vector beam (AEVB) has a salient feature that it contains a magnetic-dominant region within which electric field has a null and longitudinal magnetic field is maximum. Fresnel diffraction theory and plane-wave spectral (PWS) calculations are applied to quantify the field features of such a beam upon focusing through a lens. The diffraction-limited full width at half maximum (FWHM) of the beams longitudinal magnetic field intensity profile and complementary FWHM (CFWHM) of the beam's annular-shaped total electric field intensity profile are calculated at the lens's focal plane as a function of the lens's paraxial focal distance. Subsequently, we demonstrate, for the first time, that a very high resolution magnetic field at optical frequency with the total magnetic field FWHM of 0.23{\{}$\backslash$lambda{\}}(magnetic field spot size of 0.04{\{}$\backslash$lambda{\}}{\^{}}2) can be achieved by placing a subwavelength dense dielectric Mie scatterer in the minimum-waist plane of a self-standing converging AEVB. The theory shown here is valuable for the development of optical microscopy and spectroscopy systems based on magnetic dipolar transitions which are in general much weaker than their electric counterparts.},
author = {Veysi, Mehdi and Guclu, Caner and Capolino, Filippo},
doi = {10.1364/josab.33.002265},
file = {:C$\backslash$:/Users/DONNonlinearWS01/Desktop/PhD/Bibliography/Pool/1603.00038.pdf:pdf},
issn = {0740-3224},
journal = {Journal of the Optical Society of America B},
number = {11},
pages = {2265--2277},
title = {{Focused azimuthally polarized vector beam and spatial magnetic resolution below the diffraction limit}},
volume = {33},
year = {2016}
}
@article{Carletti2018,
author = {Carletti, Luca and Marino, Giuseppe and Ghirardini, Lavinia and Gili, Valerio F and Rocco, Davide and Favero, Ivan and Locatelli, Andrea and Zayats, Anatoly V and Celebrano, Michele and Finazzi, Marco and Giuseppe, Leo and de Angelis, Costantino and Neshev, Dragomir N.},
doi = {10.1021/acsphotonics.8b00810},
file = {:C$\backslash$:/Users/DONNonlinearWS01/AppData/Local/Mendeley Ltd./Mendeley Desktop/Downloaded/Carletti et al. - 2018 - Nonlinear goniometry by second harmonic generation in AlGaAs nanoantennas.pdf:pdf},
issn = {2330-4022},
journal = {ACS Photonics},
keywords = {all-dielectric nanoresonators,disciplines such as solid-,nanophotonics,nonlinear optics,nonlinear scattering,of,paramount importance in many,particles is a phenomenon,ptical scattering from small,radiation pattern,second-harmonic generation},
pages = {4386−4392 Article},
publisher = {American Chemical Society},
title = {{Nonlinear goniometry by second harmonic generation in AlGaAs nanoantennas}},
url = {http://pubs.acs.org/doi/10.1021/acsphotonics.8b00810},
volume = {5},
year = {2018}
}
@article{Bai2013,
abstract = {We present a semi-analytical formalism capable of handling the coupling of electromagnetic sources, such as point dipoles or freepropagating fields, with various kinds of dissipative resonances with radiation leakage, Ohmic losses or both. Due to its analyticity, the approach is very intuitive and physically-sound. It is also very economic in computational resources, since once the resonances of a plasmonic or photonic resonator are known, their excitation coefficients are obtained analytically, independently of the polarization, frequency or location of the excitation source. To evidence that the present formalism is very general and versatile, we implement it with the commercial software COMSOL, rather than with our in-house numerical tools. {\textcopyright}2013 Optical Society of America.},
author = {Bai, Q. and Perrin, M. and Sauvan, C. and Hugonin, J-P and Lalanne, P.},
doi = {10.1364/oe.21.027371},
file = {:C$\backslash$:/Users/DONNonlinearWS01/Desktop/PhD/Bibliography/Pool/Opt Express 2013 QNM computation.pdf:pdf},
journal = {Optics Express},
number = {22},
pages = {27371--27382},
title = {{Efficient and intuitive method for the analysis of light scattering by a resonant nanostructure}},
volume = {21},
year = {2013}
}
@article{Gili2016,
abstract = {We demonstrate monolithic aluminum gallium arsenide (AlGaAs) optical nanoantennas. Using a selective oxidation technique, we fabricated epitaxial semiconductor nanocylinders on an aluminum oxide substrate. Second harmonic generation from AlGaAs nanocylinders of 400 nm height and varying radius pumped with femtosecond pulses delivered at 1554-nm wavelength has been measured, revealing a peak conversion efficiency exceeding 10-5 for nanocylinders with an optimized geometry.[on SciFinder (R)]},
archivePrefix = {arXiv},
arxivId = {1604.08881},
author = {Gili, V. F. and Carletti, L. and Locatelli, A. and Rocco, D. and Finazzi, M. and Ghirardini, L. and Favero, I. and Gomez, C. and Lema{\^{i}}tre, A. and Celebrano, M. and {De Angelis}, C. and Leo, G.},
doi = {10.1364/OE.24.015965},
eprint = {1604.08881},
file = {:C$\backslash$:/Users/DONNonlinearWS01/AppData/Local/Mendeley Ltd./Mendeley Desktop/Downloaded/Gili et al. - 2016 - Monolithic AlGaAs second-harmonic nanoantennas.pdf:pdf},
issn = {1094-4087},
journal = {Optics Express},
number = {14},
pages = {15965--15971},
title = {{Monolithic AlGaAs second-harmonic nanoantennas}},
url = {https://www.osapublishing.org/abstract.cfm?URI=oe-24-14-15965},
volume = {24},
year = {2016}
}

